[MASK] is All You Need

In generative models, two paradigms have gained attraction in various applications: next-set prediction-based Masked Generative Models and next-noise prediction-based Non-Autoregressive Models, e.g., Diffusion Models. In this work, we propose using discrete-state models to connect them and explore their scalability in the vision domain. First, we conduct a step-by-step analysis in a unified design space across two types of models including timestep-independence, noise schedule, temperature, guidance strength, etc in a scalable manner. Second, we re-cast typical discriminative tasks, e.g., image segmentation, as an unmasking process from [MASK] tokens on a discrete-state model. This enables us to perform various sampling processes, including flexible conditional sampling by only training once to model the joint distribution. All aforementioned explorations lead to our framework named Discrete Interpolants, which enables us to achieve state-of-the-art or competitive performance compared to previous discrete-state based methods in various benchmarks, like ImageNet256, MS COCO, and video dataset FaceForensics. In summary, by leveraging [MASK] in discrete-state models, we can bridge Masked Generative and Non-autoregressive Diffusion models, as well as generative and discriminative tasks.

==> 6_1_append_more_details.tex <==



\section{Extra Detail}




\subsection{Training detail}

We follow the implementation of MaskGIT~\cite{chang2022maskgit} and do not use label smoothing or soft target cross-entropy. Empirically, we find that initializing the final fully connected  layer of the logits is crucial for stabilizing training, especially in multi-node setups. Gradient clipping with a norm of 2 is applied throughout the training process.  Wherever applicable, we utilize fused kernels, such as fusedAdam, to optimize performance.

In our joint training experiments, we explore various configurations of timesteps and shared vocabularies. Our findings indicate that using different timesteps with separate vocabularies consistently yields the best results.

To optimize batch size, we pre-extract the indices in advance. This approach effectively doubles the batch size in many cases. For example, on the MS COCO dataset, the maximum batch size for U-ViT2-S2-Deep on an A100-40G GPU is 28 without pre-extraction, but increases to 48 with pre-extracted indices. Additionally, in joint training, pre-tokenizing accelerates training speed significantly, improving from 1.3 iterations per second to 4.2 iterations per second with a batch size of 16.

%


\subsection{Dataset detail}


\paragraph{ImageNet256, MS COCO and Cityscapes.} We use ImageNet256 for ablation study and main comparison following previous works~\cite{uvit}. We use MS COCO 2014~\cite{coco} to explore the alignment between images and captions. For the evaluation of FID on COCO $256\times 256$, we sample prompts from the validation set, following the approach of U-ViT~\cite{uvit}.
We use the Cityscapes dataset to explore the alignment between images and segmentation. Following~\citet{hoogeboom2021argmax}, we reduce the computational cost by rescaling the segmentation maps from Cityscapes to $32\times64$ images using nearest neighbor interpolation. We utilize the global categories as prediction targets, resulting in an 8-class problem. For the real images used in FID computation, we randomly crop $256\times256$ images from the $256\times512$ landscape Cityscapes images.

\paragraph{FaceForensics.} FaceForensics contains 150×150 images of deepfake faces, totaling over 20,000 images from 1,000 videos. For video generation, we use an image-based tokenizer: SD-VQGAN~\cite{rombach2022high_latentdiffusion_ldm}. We extract 16-frame video clips from these datasets using a specific sampling interval. Each frame is resized to 256×256 resolution for training, resulting in a size of 16×3×256×256.  %















